X-VARS: Introducing Explainability in Football Refereeing with Multi-Modal Large Language Model

The rapid advancement of artificial intelligence has led to significant improvements in automated decision-making. However, the increased performance of models often comes at the cost of explainability and transparency of their decision-making processes. In this paper, we investigate the capabilities of large language models to explain decisions, using football refereeing as a testing ground, given its decision complexity and subjectivity. We introduce the Explainable Video Assistant Referee System, X-VARS, a multi-modal large language model designed for understanding football videos from the point of view of a referee. X-VARS can perform a multitude of tasks, including video description, question answering, action recognition, and conducting meaningful conversations based on video content and in accordance with the Laws of the Game for football referees. We validate X-VARS on our novel dataset, SoccerNet-XFoul, which consists of more than 22k video-question-answer triplets annotated by over 70 experienced football referees. Our experiments and human study illustrate the impressive capabilities of X-VARS in interpreting complex football clips. Furthermore, we highlight the potential of X-VARS to reach human performance and support football referees in the future.

==> deleted.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.45\linewidth]{figures/Dataset/views_image1.png}
  \includegraphics[width=0.45\linewidth]{figures/Dataset/views_image2.png}
            \caption{ \textbf{Multi-view action}. Left: 'Live action clips' refer to all the clips taken from the main camera. Right: 'Replay clips' refer to all the clips taken by another camera.}\label{action_views}
\end{figure}


\textbf{Severity of different foul classes}
The distribution of the severity among different foul classes can provide insight into how often certain types of fouls result in a card being shown to the offending player.\\

In the figure \ref{severity_per_foul}, we can see that the action classes 'challenge' and 'pushing' have a high percentage of the foul being 'no card' with 87,9\%, respectively 93,8\%. 
Only in very few cases a foul of one of these classes has as consequence a 'yellow card'.\\

On the other hand, some classes are inseparably with an immediate yellow card. Especially, the 'high leg' class (53,2\%), the 'tackling class' (46,2\%) and 'illegal use of arms' class (39,1\%) are the foul classes for which a player will receive often a 'yellow card'. 
All these classes represents fouls for which the player acts with disregard to the danger for an opponent.
It is not surprising that these classes also have a higher likelihood of resulting in a 'red card', with 'high leg' (4,8\%), 'illegal use of arms' (2,3\%) and 'tackling' (3,5\%) having the highest percentage of 'red cards'.

\begin{figure}[htbp]
  \centering
  \includegraphics[width=1\linewidth]{figures/Dataset/severity_per_foul.png}
            \caption{The severity distribution for the different action classes}
        \label{severity_per_foul}
\end{figure}

==> figures/ellbow_yellow.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{pictures/Ellbow Yellow.png}
\caption{
\textbf{Qualitative results.} 
}
\label{}
\end{figure*}

==> figures/high_leg_red_card.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{pictures/High_leg_red_card.png}
\caption{
\textbf{Qualitative results.} What card would you give and why? 
Video-ChatGPT: Based on the video, I would give the player a yellow card for unsportsmanlike conduct. The player was seen kicking the ball into the goalkeeper’s face, which is not a fair or respectful play.
}
\label{importance of the views}
\end{figure*}

==> figures/pipeline.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{pictures/Pipeline.png}
\caption{
\textbf{Architecture of VARS-Ex.} 
}
\label{fig:pipeline}
\end{figure*}

==> figures/supp_qualitative_results.tex <==
\begin{figure}
  \centering
  \includegraphics[width=1\linewidth]{pictures/Tackling_Yellow_Discussion.png}
\caption{
\textbf{Qualitiative results.} 
}
\label{fig:supp_qual_tackling}
\end{figure}

==> figures/tackling_red_card.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{pictures/Unbenannt.png}
\caption{
\textbf{Qualitative results.} 
}
\label{}
\end{figure*}

==> figures/tackling_yellow.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth]{pictures/Tackling Yellow.png}
\caption{
\textbf{Qualitative results.} 
}
\label{}
\end{figure*}

==> tables/quantitative_results.tex <==
\begin{table}
\centering
\setlength{\extrarowheight}{4pt}
\begin{tabular}{c|cc}
  &Mean &Std \\
\hline
Referees &4.0 &1.0 \\
X-VARS &3.8 &1.1 \\

\end{tabular}
\caption{ \textbf{Quantitative results.} 
The mean scores of X-VARS closely match those of human referees. 
In 46\% of the video clips, X-VARS achieved higher scores than the human referees. 
A score of 5 is the highest and represents \textit{strongly agree}, with "Std" denoting the standard deviation.
}
    \label{tab:quantitative}
\end{table}



==> tables/training_parameters_stage_1.tex <==
\begin{table}
\centering
\setlength{\extrarowheight}{4pt}
\begin{tabular}{c|c}
\textbf{Hyperparameters} & \\
\hline
Batch size & 64 \\
Data augmentation & Yes \\
\#Frames & 16 \\
Frame resolution & 224x224p\\
Scheduler & Step \\
LR & 5e-6 \\
Step & 8 \\
Gamma & 0.8 \\
Weight decay & 0.01 \\
Optimizer & AdamW \\
GPU & Nvidia A100 16GB

\end{tabular}
\caption{Hyperparameters of training stage 1.
Data augmentation was performed with RandomRotation, RandomAffine, RandomPerspective, ColorJitter, RandomHorizontalFlip. 
}
    \label{tab:training_parameters_stage_1}
\end{table}


==> tables/training_parameters_stage_2.tex <==
\begin{table}
\centering
\setlength{\extrarowheight}{4pt}
\begin{tabular}{c|c}
\textbf{Hyperparameters} &  \\
\hline
Batch size & 32 \\
\#Frames & 16 \\
Frame resolution & 224x224p\\
Scheduler & Constant \\
LR & 2e-4 \\
Weight decay & 0.001 \\
Optimizer & AdamW \\
GPU & 2 Nvidia A100 40GB

\end{tabular}
\caption{Hyperparameters of training stage 2.
}
    \label{tab:training_parameters_stage_2}
\end{table}

